Meta-prediction Model for Distillation-Aware NAS on Unseen Datasets

Distillation-aware Neural Architecture Search (DaNAS) aims to search for an optimal student architecture that obtains the best performance and/or efficiency when distilling the knowledge from a given teacher model. Previous DaNAS methods have mostly tackled the search for the neural architecture for fixed datasets and the teacher, which are not generalized well on a new task consisting of an unseen dataset and an unseen teacher, thus need to perform a costly search for any new combination of the datasets and the teachers. For standard NAS tasks without KD, meta-learning-based computationally efficient NAS methods have been proposed, which learn the generalized search process over multiple tasks (datasets) and transfer the knowledge obtained over those tasks to a new task. However, since they assume learning from scratch without KD from a teacher, they might not be ideal for DaNAS scenarios. To eliminate the excessive computational cost of DaNAS methods and the sub-optimality of rapid NAS methods, we propose a distillation-aware meta accuracy prediction model, DaSS (Distillation-aware Student Search), which can predict a given architecture's final performances on a dataset when performing KD with a given teacher, without having actually to train it on the target task. The experimental results demonstrate that our proposed meta-prediction model successfully generalizes to multiple unseen datasets for DaNAS tasks, largely outperforming existing meta-NAS methods and rapid NAS baselines. Code is available at https://github.com/CownowAn/DaSS

==> Algorithm/algorithm.tex <==
\begin{minipage}{.50\linewidth}
\begin{algorithm}[H]
	\caption{Meta-training}\label{algo:algorithm1}
	\small
	\begin{algorithmic}[1]
		\State \textbf{Input:} $(\D_1, \tilde{\theta}_1),\dots,(\D_T, \tilde{\theta}_T)$
		\State \textbf{Input:} Architecture Set $\mathcal{S}$
		\State \textbf{Input:} Learning rate $\alpha$, $\beta$
		\State \textbf{Output:} $\phi^*$
		\State Randomly initialize $\phi$
		\While{not converged}
% 		\State $\mathcal{L}^\te \leftarrow 0$
		\For{$t=1$ to $T$}
		\State Sample $s \sim \mathcal{S}$.
        \State Sample batches $\{\mathcal{B}_t\} \sim \D_t$ 
		\State Compute $w = f(\tilde{\theta}_t, s; \phi)$.
		\State Remap $\theta_t = w * \tilde{\theta}_t$.
		\State Compute $\mathcal{L}(\mathcal{B}_t;s, \theta_t,\phi)$.
		\EndFor
		\State $\phi \leftarrow \phi - \beta \grad_{\phi} \frac{1}{T}\sum_{t=1}^{T} \mathcal{L}(\mathcal{B}_t;s, \theta_t,\phi)$
		\EndWhile
	\end{algorithmic}
	\end{algorithm}
\end{minipage}
\begin{minipage}{.50\linewidth}
\begin{algorithm}[H]
	\caption{Meta-test}\label{algo:algorithm2}
	\small
	\begin{algorithmic}[1]
		\State \textbf{Input:} $\D, \D^{te} \tilde{\theta}, \phi^*$
		\State \textbf{Input:} Architecture Set $\mathcal{S}$
		\State \textbf{Input:} Learning rate $\alpha$
		\State \textbf{Output:} $\theta^*$
		\While{not converged}
		\State Sample $s \sim \mathcal{S}$.
        \State Sample batches $\{\mathcal{B}\} \sim \D$ 
		\State Compute $w = f(\tilde{\theta}, s; \phi^*)$.
		\State Remap $\theta = w * \tilde{\theta}$.
		\EndWhile
		\State Evaluate the test examples in  $\D^{te}$ with the parameter $\theta^*$ and architecture $s$.
	\end{algorithmic}
	\end{algorithm}
\end{minipage}


==> Figure/PR.tex <==
\begin{wrapfigure}{r}{0.4\textwidth}
\vspace{-0.15in}
    \small
    \centering
    \includegraphics[width=0.4\textwidth]{Figure/PR.pdf} 
    \vspace{-0.10in}
    \resizebox{1.\linewidth}{!}{
    \caption{\small \textbf{Parameter Remapping}
    }
    \label{fig:PR}
    \vspace{-0.15in}
    }
\end{wrapfigure}



% \begin{wraptable}{r}{0.4\textwidth}
% \vspace{-0.15in}
% \caption{\small Comparison between accuracy prediction models for NAS and DaNAS.}\label{tbl:comparison}
% \vspace{-0.2in}
% \resizebox{1.\linewidth}{!}{
% \begin{tabular}{ccccc}\\\toprule  
% \small
% & Task-spec. & MetaD2A & TANS & \textbf{Ours} \\
% \midrule
% Time Compl. & $O(N)$ & $O(1)$  & $O(1)$  & \textbf{$O(1)$}\\  
% \midrule

% Meta-learning & \textsf{X}  & \textsf{O} & \textsf{O} & \textbf{\textsf{O}}\\  

% \midrule
% Unseen Arch. & \textsf{O} & \textsf{O} & \textsf{O} & \textbf{\textsf{O}}\\  

% \midrule
% Unseen Data. & \textsf{X} & \textsf{O} & \textsf{O} &\textbf{\textsf{O}}\\ 
% \midrule
% Unseen Teach. & \textsf{X} & \textsf{X} & \textsf{X} & \textbf{\textsf{O}}\\  

% \midrule
% Distil.-aware & \textsf{X} & \textsf{X} & \textsf{X} & \textbf{\textsf{O}}\\  
% \midrule
% Fast Adapt. & \textsf{X} & \textsf{X} & \textsf{X} & \textbf{\textsf{O}}\\  
% \bottomrule
% \vspace{-0.3in}
% \end{tabular}
% }
% \end{wraptable} 

==> Figure/fig_2_meta_learning.tex <==
\begin{figure*}[t]
    \small
    \centering
    \vspace{-0.05in}
    \includegraphics[width=0.98\textwidth]{Figure/fig_meta_learning.pdf} 
    \vspace{-0.1in}
    \caption{\small \textbf{Distillation-aware Meta-learning.} \small 
    To search for the optimal student architecture to distill the knowledge from the given teacher network $\mathbf{t}( \cdot; \bm{\tilde{\theta}})^\tau$ well, the sampled task should be encoded in a distillation-aware way. By taking a fixed input after remapping the trained parameters of teacher to the randomly sampled student candidate, we can encode the student candidate functionally in a teacher-adaptive way. Along with the functional embedding, by considering the architecture configuration of the student, we encode sampled task in a way appropriate for the distillation-aware NAS.
    Also, one-shot adaptation with teacher embedding which contains both architectural and functional information makes teacher-guided meta-learning becomes possible.
    }
    \label{fig:meta-learning}
    \vspace{-0.15in}
\end{figure*}


==> Figure/fig_3_transfer_unseen.tex <==
\begin{figure*}[t]
    \small
    \centering
    \includegraphics[width=0.98\textwidth]{Figure/fig_transfer_unseen.pdf} 
    \vspace{-0.10in}
    \caption{\small \textbf{Transfer to Unseen Task.} \small 
    With transferred meta-knowledge $\phi^{*}$ learned from meta training, our meta-predictor $f(\cdot;\phi^{*})$ can adapt to an unseen task $\hat{\tau}$. Especially, inner updating our meta-prediction model through a teacher network-accuracy pair, which is referred as the teacher-guide, the adaptation can be conducted quickly with almost no cost. Then, by remapping parameters of teacher network trained on $\bf{D}^{\tau}$ to the given student candidate, teacher-adaptive embedding of the student candidate can be obtained. Utilizing this teacher-aware embedding scheme, our meta-prediction model can rapidly output estimated distillation performance of the given student architecture on the unseen task.
    }
    \label{fig:transfer_unseen}
    \vspace{-0.15in}
\end{figure*}

==> Figure/fig_4_efficiency_figure.tex <==
% \begin{figure}[t]
%     \vspace{-0.1in}
% 	\centering
% 	\subfigure[CUB]{
% 	\includegraphics[width=3.1cm]{Figure/cub_time.pdf}
% 	\label{fig:cub_time}
% 	}
% 	\subfigure[SFD]{
% 	\includegraphics[width=3.1cm]{Figure/sfd_time.pdf}
% 	\label{fig:sfd_time}
% 	}
% 	\subfigure[DTD]{
% 	\includegraphics[width=3.1cm]{Figure/dtd_time.pdf}
% 	\label{fig:dtd_time}
% 	}
% 	\subfigure[STL]{
% 	\includegraphics[width=3.1cm]{Figure/stl_time.pdf}
% 	\label{fig:stl_time}
% 	}
% 	\vspace{-0.1in}
% 	\caption{\small \textbf{Collecting time} }
% 	\vspace{-0.05in}
% \end{figure}

\begin{figure}[t]
    % \vspace{-0.05in}
	\centering
% 	\vspace{-0.15in}
	\caption{\small \textbf{Time and Sample Efficiency of the Proposed Meta-prediction Model for DaNAS} \small Comparison of
the time required to collect samples for adaptation in guided search.  The \textbf{Collecting time} refers to the time required to obtain architecture-performance pairs (\textbf{Number of samples}) in the guided meta-learning strategy. Our one-shot adaptation guided search with the teacher network which is already trained under the DaNAS task is much more efficient than utilizing a few-shot adaptation with a few student architecture-accuracy pair(s).}
	\vspace{-0.1in}
	\subfigure[CUB]{
	\includegraphics[width=2.9cm]{Figure/cub_time.pdf}
	\label{fig:cub_time}
	}
	\subfigure[Stanford Cars]{
	\includegraphics[width=2.9cm]{Figure/sfc_time.pdf}
	\label{fig:sfd_time}
	}
	\subfigure[DTD]{
	\includegraphics[width=2.9cm]{Figure/dtd_time.pdf}
	\label{fig:dtd_time}
	}
	\subfigure[STL]{
	\includegraphics[width=2.9cm]{Figure/stl_time.pdf}
	\label{fig:stl_time}
	}
% 	\subfigure[SFD]{
% 	\includegraphics[width=1.4cm]{Figure/sfd_time.pdf}
% 	\label{fig:sfd_time}
% 	}
% 	\subfigure[SFD]{
% 	\includegraphics[width=1.4cm]{Figure/sfd_time.pdf}
% 	\label{fig:sfd_time}
% 	}
% 	\subfigure[SFD]{
% 	\includegraphics[width=1.4cm]{Figure/sfd_time.pdf}
% 	\label{fig:sfd_time}
% 	}
% 	\subfigure[SFD]{
% 	\includegraphics[width=1.4cm]{Figure/sfd_time.pdf}
% 	\label{fig:sfd_time}
% 	}
	\vspace{-0.15in}
% 	\caption{\small \textbf{Time and Sample Efficiency} The \textbf{collecting time for Ours (student)} refers to the time required to obtain several (architecture-performance) pairs in the guided meta-learning strategy. The \textbf{Number of samples} means the number of these pairs. In order to obtain one pair, knowledge distillation for each network must be performed until fully converged, and then performance should be obtained. With the (architecture-performance) pair of the teacher network as we suggested, the collecting time requires only one forward time to obtain the teacher’s performance ( (\textbf{collecting time for Ours (teacher)}).}
	\label{fig:time}
	\vspace{-0.1in}
\end{figure}

==> Table/tbl_final_corr.tex <==
\begin{table*}[t!]
	\caption{\small \textbf{Comparison with Rapid NAS Methods. / End-to-end AKD} }
	\vspace{-0.15in}
	\small
	\begin{center}
     \resizebox{\linewidth}{!}{
	    \begin{tabular}{cl|cccccc}
	   	\toprule
	   	\multicolumn{2}{c|}{\multirow{2}{*}{Method}} & 
	   	\multicolumn{6}{c}{Correlation}           \\
                                                         &
                                                         &
	      CUB                                          &
            Stanford Dogs                                &
            DTD                                          & 
            CIFAR-10                                     &
	      CIFAR-100                                    & 
	    STL10                                       \\
	   	\midrule
	   	\midrule
                                                             &
	    \multicolumn{1}{l|}{Params}                      &
            -0.076                                             &
            0.008                                             &
            0.026                                             &
            0.323                                             &
            0.422                                             &
            -0.054                                             \\
                                                             &
	    \multicolumn{1}{l|}{FLOPs}                       &
            0.101                                             &
            0.318                                             &
            0.100                                             &
            0.552                                             &
            0.544                                             &
            -0.145                                             \\
	   	\midrule  
                                                             &
	   	\multicolumn{1}{l|}{grad norm~\citep{abdelfattah2021zero}}                   &
            -0.086                                             &
             0.170                                             &
            0.164                                             &
            0.034                                            &
            0.365                                             &
            0.190                                             \\
                                                             &
	   	\multicolumn{1}{l|}{snip~\citep{abdelfattah2021zero}}                        &
            0.147                                             &
            0.339                                             &
            0.223                                             &
            0.218                                             &
            0.486                                             &
            0.333                                             \\
                                                             &
	   	\multicolumn{1}{l|}{grasp~\citep{abdelfattah2021zero}}                       &
            -0.099                                             &
            -0.041                                             &
            -0.068                                             &
            -0.300                                             &
            -0.416                                             &
            0.166                                             \\
            Zero-cost                                        &
	    \multicolumn{1}{l|}{fisher~\citep{abdelfattah2021zero}}                      &
            0.037                                             &
            0.103                                             &
            0.257                                             &
            -0.088                                             &
            0.158                                             &
            0.176                                             \\
            Proxies                                          &
	    \multicolumn{1}{l|}{jacob cov~\citep{abdelfattah2021zero}}                   &
            -0.251                                             &
            0.138                                             &
            0.110                                             &
            0.629                                             &
            0.360                                             &
            0.379                                             \\
                                                             &
	    \multicolumn{1}{l|}{plain~\citep{abdelfattah2021zero}}                       &
            0.191                                             &
            0.255                                             &
            0.302                                             &
            -0.045                                             &
            0.406                                             &
            0.246                                             \\
                                                             &
            \multicolumn{1}{l|}{synflow bn~\citep{abdelfattah2021zero}}                     &
            -0.180                                             &
            0.224                                             &
            0.028                                             &
            0.364                                             &
            0.468                                             &
            0.431                                             \\
                                                             &                     
	    \multicolumn{1}{l|}{synflow~\citep{abdelfattah2021zero}}                     &
            -0.017                                             &
            0.347                                             &
            0.181                                             &
            0.395                                             &
            0.304                                             &
            0.307                                             \\
                                                             &
	    \multicolumn{1}{l|}{NASWOT~\citep{mellor2021neural}}                      &
            x.xx                                             &
            x.xx                                             &
            x.xx                                             &
            x.xx                                             &
            x.xx                                             &
            x.xx                                             \\
	    \midrule
            \multirow{2}{*}{Meta-learning}                   &
	    \multicolumn{1}{l|}{TANS~\citep{jeong2021task}}  &
            x.xx                                             &
            x.xx                                             &
            x.xx                                             &
            x.xx                                             &
            x.xx                                             &
            x.xx                                             \\
                                                             &
	   	\multicolumn{1}{l|}{MetaD2A~\citep{lee2021rapid}}&       	
            x.xx                                             &
            x.xx                                             &
            x.xx                                             &
            x.xx                                             &
            x.xx                                             &
            x.xx                                             \\
	    \midrule
            
            \multirow{1}{*}{Ours}                   &         
	    \multicolumn{1}{l|}{\multirow{1}{*}{\textbf{Meta-learning}}} &
	    \textbf{0.731}                                       &
	    \textbf{0.578}	   		   	                        &
	    \textbf{0.401}                                       &
	    \textbf{0.374}                                       &
	    \textbf{0.404}                                       &
	    \textbf{0.320}                                      \\
	   	\bottomrule
        \end{tabular}}
	\end{center}
	\small
	\label{tbl:final}	
\end{table*}




==> Table/tbl_final_corr_spearmanr.tex <==
\begin{table*}[t!]
	\caption{\small \textbf{Comparison with Rapid NAS Methods. / End-to-end AKD} }
	\vspace{-0.15in}
	\small
	\begin{center}
     \resizebox{\linewidth}{!}{
	    \begin{tabular}{cl|cccccc}
	   	\toprule
	   	\multicolumn{2}{c|}{\multirow{2}{*}{Method}} & 
	   	\multicolumn{6}{c}{Correlation}           \\
                                                         &
                                                         &
	      CUB                                          &
            Stanford Dogs                                &
            DTD                                          & 
	      CIFAR-100                                    & 
	    STL10                                       \\
	   	\midrule
	   	\midrule
                                                             &
	    \multicolumn{1}{l|}{Params}                      &
            -0.076                                             &
            0.008                                             &
            0.323                                             &
            0.422                                             &
            -0.054                                             \\
                                                             &
	    \multicolumn{1}{l|}{FLOPs}                       &
            0.101                                             &
            0.318                                             &
            0.552                                             &
            0.544                                             &
            -0.145                                             \\
	   	\midrule  
                                                             &
	   	\multicolumn{1}{l|}{grad norm~\citep{abdelfattah2021zero}}                   &
            -0.066                                             &
             0.201                                             &
            0.188                                             &
            0.378                                             &
            0.218                                             \\
                                                             &
	   	\multicolumn{1}{l|}{snip~\citep{abdelfattah2021zero}}                        &
            0.108                                             &
            0.289                                             &
            0.235                                             &
            0.416                                             &
            0.397                                             \\
                                                             &
	   	\multicolumn{1}{l|}{grasp~\citep{abdelfattah2021zero}}                       &
            -0.153                                             &
            -0.095                                             &
            -0.187                                             &
            -0.381                                             &
            -0.101                                             \\
            Zero-cost                                        &
	    \multicolumn{1}{l|}{fisher~\citep{abdelfattah2021zero}}                      &
            0.028                                             &
            -0.026                                             &
            0.199                                             &
            0.276                                             &
            0.271                                             \\
            Proxies                                          &
	    \multicolumn{1}{l|}{jacob cov~\citep{abdelfattah2021zero}}                   &
            -0.454                                             &
            0.197                                             &
            0.323                                             &
            0.270                                             &
            0.288                                             \\
                                                             &
	    \multicolumn{1}{l|}{plain~\citep{abdelfattah2021zero}}                       &
            0.124                                             &
            0.179                                             &
            0.260                                             &
            0.356                                             &
            0.342                                             \\
                                                             &
            \multicolumn{1}{l|}{synflow bn~\citep{abdelfattah2021zero}}                     &
            -0.096                                             &
            0.273                                             &
            0.165                                             &
            0.479                                             &
            0.501                                             \\
                                                             &                     
	    \multicolumn{1}{l|}{synflow~\citep{abdelfattah2021zero}}                     &
            -0.033                                             &
            0.304                                             &
            0.273                                             &
            0.481                                             &
            0.522                                             \\
                                                             &
	    \multicolumn{1}{l|}{NASWOT~\citep{mellor2021neural}}                      &
            x.xx                                             &
            x.xx                                             &
            x.xx                                             &
            x.xx                                             &
            x.xx                                             \\
	    \midrule
            \multirow{2}{*}{Meta-learning}                   &
	    \multicolumn{1}{l|}{TANS~\citep{jeong2021task}}  &
            x.xx                                             &
            x.xx                                             &
            x.xx                                             &
            x.xx                                             &
            x.xx                                             \\
                                                             &
	   	\multicolumn{1}{l|}{MetaD2A~\citep{lee2021rapid}}&       	
            x.xx                                             &
            x.xx                                             &
            x.xx                                             &
            x.xx                                             &
            x.xx                                             \\
	    \midrule
            
            \multirow{1}{*}{Ours}                   &         
	    \multicolumn{1}{l|}{\multirow{1}{*}{\textbf{Meta-learning}}} &
	    \textbf{0.780}                                       &
	    \textbf{0.510}	   		   	                        &
	    \textbf{0.476}                                       &
	    \textbf{0.406}                                       &
	    \textbf{0.485}                                      \\
	   	\bottomrule
        \end{tabular}}
	\end{center}
	\small
	\label{tbl:final}	
\end{table*}




==> Table/tbl_final_end2end.tex <==
% \begin{table*}[t!]
% 	\vspace{-0.1in}
% 	\small
% 	\begin{center}
%      \resizebox{\linewidth}{!}{
% 	    \begin{tabular}{cccccccccccc}
% 	   	\toprule
%                              &
%      	\multicolumn{10}{c}{Method}           &
%             \multicolumn{1}{c}{\multirow{2}{*}{Teacher}} \\
% 	   	                                           &
% 	   	grad norm                                         &
%         snip                                              &
%         grasp                                             &
% 	    fisher                                            &
%         jacob cov                                         &
%         plain                                             & 
%         synflow                                           &
% 	    TANS                                              & 
% 	    MetaD2A                                          &
% 	    \textbf{Ours}                                                \\
% 	    \hline
% 	    \midrule
%          CUB   	                                            &
% 	17.26                                            &
%         17.26                                         &
%         19.86                                            &
% 	17.26                                          &
%         23.33                                          &
%         21.89                                          & 
%         16.72                                 &
% 	22.83                                    & 
% 	  22.59                                         &
% 	\textbf{23.85}                                 &
%         23.30                                         \\
%  %         SfD   	                                            &
% 	% 15.22                                            &
%  %    29.92                                         &
%  %    18.46                                            &
% 	% 24.65                                          &
%  %    30.81                                     &
%  %    30.82                                          & 
%  %    14.67                                     &
% 	% 27.18                                    & 
% 	% 28.91                                         &
% 	% \textbf{25.72}                                 &
%  %        31.44                                         \\
%  %        C100   	                                            &
% 	% 55.75                                            &
%  %        56.88                                     &
%  %        58.48                                        &
% 	% 53.23                                          &
%  %        58.50                                     &
%  %        53.59                                          & 
%  %        54.25                                     &
% 	% 56.65                                         &
%  %        57.52                                    & 
% 	% \textbf{58.73}                                 &
%  %        74.09                                         \\
%         SFC   	                                            &
% 	29.89                                           &
%         29.89                                     &
%         11.19                                        &
%         29.89                                          &
%         34.30                                     &
%         29.89                                     &
%         23.16                                          & 
% 	27.60                                         &
%         30.53                                    & 
% 	\textbf{34.79}                                 &
%         62.70                                         \\
% 	   STL                                        &
% 	   	41.34                                            &
%         41.34                                            &
%         36.16                                            &
% 	    49.86                                          &
%         44.59                                          &
%         41.34                                          & 
%         36.44                                     &
% 	    47.23                                    & 
% 	    43.25                                         &
% 	    \textbf{50.00}                                 &
%             70.77                                         \\
%          DTD   	                                            &
% 	   	16.16                                            &
%         16.16                                         &
%         16.16                                            &
% 	12.82                                          &
%         14.33                                          &
%         16.54                                          & 
%         14.98                                     &
% 	12.82                                    & 
% 	    17.89                                         &
% 	    \textbf{19.23}                                 &
%             21.44                                         \\
% 	   	\bottomrule
%         \end{tabular}}
% 	\end{center}
% 	\small
% 	\vspace{-0.15in}
% 	\caption{\small \textbf{End-to-end Distillation-aware NAS} }
% 	\label{tbl:final}
% 	\vspace{-0.25in}
% \end{table*}



\begin{table*}[t!]
	\vspace{-0.05in}
	\small
	\caption{\small \textbf{End-to-end Distillation-aware NAS on Unseen Datasets} We randomly sample 10,000 student architectures and select the top-1 student architecture whose estimated performance by each method is the highest, and then distill the knowledge from the same teacher network trained on the target dataset to the selected student architecture with the same number of epochs. We report the final accuracy of each distilled student.}  	
	\vspace{-0.2in}
	\begin{center}
     \resizebox{\linewidth}{!}{
	    \begin{tabular}{cccccccccccc}
	   	\toprule
                             &
     	\multicolumn{10}{c}{Method}           &
            \multicolumn{1}{c}{\multirow{2}{*}{Teacher}} \\
	   	                                           &
	   	grad norm                                         &
        snip                                              &
        grasp                                             &
	    fisher                                            &
        plain                                             & 
        synflow                                           &
        NASWOT                                         &
	    MetaD2A                                              & 
	    TANS                                          &
	    \textbf{Ours}                                                \\
	    \hline
	    \midrule
         CUB   	                                            &
	    17.26                                            &
        17.26                                         &
        19.86                                            &
	    17.26                                          &
        21.89                                          & 
        16.72                                 &
        23.33                                          &
	    22.59                                         &
	    22.83                                    & 
	\textbf{23.85}                                 &
        23.30                                         \\
        SFC   	                                            &
	    29.89                                           &
        29.89                                     &
        11.19                                        &
        29.89                                          &
        29.89                                     &
        23.16                                          & 
        34.30                                     &
        30.53                                    & 
        27.60                                         &
	\textbf{34.79}                                 &
        62.70                                         \\
	   STL                                        &
	   	41.34                                            &
        41.34                                            &
        36.16                                            &
	    49.86                                          &
        41.34                                          & 
        36.44                                     &
        44.59                                          &
	    43.25                                         &
	    47.23                                    & 
	    \textbf{50.00}                                 &
            70.77                                         \\
         DTD   	                                            &
	   	16.16                                            &
        16.16                                         &
        16.16                                            &
	    12.82                                          &
        16.54                                          & 
        14.98                                     &
        14.33                                          &
	    17.89                                         &
	    12.82                                    & 
	    \textbf{19.23}                                 &
            21.44                                         \\
	   	\bottomrule
        \end{tabular}}
	\end{center}
	\small
	\vspace{-0.15in}
	
	\label{tbl:final}
	\vspace{-0.1in}
\end{table*}




% \begin{table*}[t]
%     \begin{center}
%   		\caption{\small \textbf{Comparison with Rapid proxies for the NAS Problem} %Spearman's Rank Correlation.} 
% 		\label{tbl:efficacy_baseline2}	}
%     \vspace{-0.1in}
%     % \label{tbl:ofa}
    
%     \resizebox{\linewidth}{!}{
    
%             \begin{tabular}{clccccccccc|c}
%              \toprule
%              \centering
% 	   	                                            &
% 	   	 & 
% 	     &
%         \\
% 	   	                                             &
%                                                      &
%             CUB                                      &
% 	        SfC                                      &
% 	        DTD                                      &
%             STL                                      &
% 	        Mean                                     &
%             CUB                                      &
% 	        SfC                                      &
% 	        DTD                                      &
%             \multicolumn{1}{c|}{\multirow{1}{*}{\textbf{Mean}}}  &
%             \multicolumn{1}{c}{\multirow{1}{*}{\textbf{Mean}}}  \\
%              \midrule
%              \midrule
%                                                             &
% 	   	 &
%             0.11                                             &
%             0.27                                             &
%             0.24                                             &
%             % 0.218                                             &
%             % 0.48                                             &
%             0.40                                             &
%             0.26                                                &
%             1.05                                                   &    
%             0.97                                             &    
%             0.97                                             &
%             \multicolumn{1}{c|}{\multirow{1}{*}{\textbf{2.14}}}                                  &
%             1.28                                            \\
%                                                             &
% 	    &
%             -0.15                                             &
%             -0.06                                             &
%             -0.19                                             &
%             % -0.300                                             &
%             % -0.41                                             &
%             -0.10                                             &
%             -0.13                                                &
%             1.37                                               &    
%             1.34                                             &    
%             1.34                                             &
%             2.56                                             &
%             1.65                                            \\
%             Zero-cost                                          &
% 	   &
%             0.03                                             &
%             0.08                                             &
%             0.20                                             &
%             % -0.088                                             &
%             % 0.15                                             &
%             0.27                                              &
%             0.11                                               &    
%             0.97                                               &    
%             0.98                                             &    
%             1.05                                             &
%             2.10                                             &
%             1.28                                            \\
%             proxies                                                &
% 	    % \multicolumn{1}{l|}{jacob cov~\citep{mellor2021neural}}&
%      %        -0.45                                             &
%      %        0.15                                             &
%      %        0.32                                             &
%      %        % 0.629                                             &
%      %        % 0.36                                             &
%      %        0.29                                              &
%      %        0.09                                              &
%      %        0.92                                             &    
%      %        0.95                                             &    
%      %        1.02                                             &
%      %        2.03                                             &
%      %        1.23                                            \\
%      %                                                         &
% 	    &
%             0.12                                             &
%             0.22                                             &
%             0.26                                             &
%             % -0.045                                             &
%             % 0.40                                             &
%             0.34                                              &
%             0.22                                              &
%             0.90                                            &    
%             0.97                                             &    
%             1.03                                             &
%             2.10                                             &
%             1.25                                            \\

%                                                              &
%             &
%             -0.10                                             &
%             0.13                                             &
%             0.17                                             &
%             % 0.364                                             &
%             % 0.46                                             &
%             \textbf{0.50}                                     &
%             0.21                                              & 
%             0.85                                             &    
%             0.97                                             &    
%             0.97                                             &
%             2.16                                             &
%             1.24                                            \\   
%             &
%             &
%             -0.45                                             &
%             0.15                                             &
%             0.32                                             &
%             % 0.629                                             &
%             % 0.36                                             &
%             0.29                                              &
%             0.09                                              &
%             0.92                                             &    
%             0.95                                             &    
%             1.02                                             &
%             2.03                                             &
%             1.23                                            \\
% 	    %\midrule
%                              &
%         % \multicolumn{3}{c}{Meta-learning}  &
% 	   &
%             0.44                                             &
%             0.44                                             &
%             0.13                                             &
%             % -0.045                                             &
%             % 0.40                                             &
%             0.09                                              &
%             0.20                                                &
%             0.01                                               &    
%             0.01                                             &    
%             0.01                                             &
%             0.01                                             &
%             0.01                                            \\
%             \midrule

%              \bottomrule
%              \end{tabular}
            
%         %     
%             }
            
%     \end{center}
%     \vspace{-0.2in}
% \end{table*}% \begin{table}[t]

==> Table/tbl_teacher.tex <==
\begin{wraptable}{r}{0.43\textwidth}
\vspace{-0.15in}
\caption{\small \textbf{{The Effect of Teacher-aware NAS}}}
\vspace{-0.1in}
\resizebox{0.43\textwidth}{!}{
%\vspace{-0.15in}
	\begin{tabular}{l|cc}
			\toprule
			\multicolumn{1}{l}{} & Teacher 1 (T1) &  Teacher 2 (T2)  \\
			\midrule
			\midrule
% 			MAML~\citep{finn2017model}
% 			& 32.9
% 			& 48.70
% 			\\
% 	        MAML++~\citep{antoniou2018train}
% 			& 32.9
% 			& 52.15
% 			\\
% 			\midrule
	        \multicolumn{1}{l}{Student for T1}
			& 65.76
			& 71.04
			\\
	        \multicolumn{1}{l}{Student for T2}
			& 65.69
			& 72.19
			\\
			\bottomrule
		\end{tabular} 
	  }
\vspace{-0.1in}
\label{tbl:teacher}
\end{wraptable}


==> Table/tbl_time.tex <==

% \begin{table*}[t!]
% 	\vspace{-0.05in}
% 	\small
% 	\caption{\small \textbf{Time and Sample Efficiency of the Proposed Meta-prediction Model for DaNAS} Comparison of the time required to collect samples for adaptation in guided search. Our one-shot adaptation guided search with the teacher network which is already trained under the DaNAS task is much more efficient than utilizing a few-shot adaptation with a few student architecture-accuracy pair(s). } %  45797/30152 GPU seconds
% 	\label{tbl:time}
% 	\vspace{-0.15in}
% 	\begin{center}
%      \resizebox{\linewidth}{!}{
% 	    \begin{tabular}{clccccc}
% 	   	\toprule
% 	   	\multirow{2}{*}{Target Dataset}                     &
% 	   	\multicolumn{1}{c}{\multirow{2}{*}{Method}}         & 
% 	   	\multicolumn{1}{c}{\multirow{2}{*}{Corr.}}    &
%         \multicolumn{4}{c}{Training}                 \\
% 	   	                                                & 
% 	   	                                                &
% 	                                                    & 
%             Sample Type                                 &
% 	      \# of Samples                                 & 
% 	   	  Collecting Time                                 & 
% 	      Speed Up	                                  \\
% 	   	\midrule
% 	   	\midrule
% %%%%%%%%%%%%%%%%%%%%%%%%   CUB  %%%%%%%%%%%%%%%%%%%%%%%%%
% %             \multirow{6}{*}{CUB}                  &
% %             % \multicolumn{1}{c|}{\multirow{6}{*}{CIFAR-10}}                  &
% % 	   	\multirow{2}{*}{Task-specific predictor}   &
% % 	   	x.xxx                                      &
% % 	   	Student                                    &
% % 	   	xxx                                        &
% % 	    xxx (s)	                                   &
% % 	      xxx$\times$                                \\
% %                                                         &
% %                                                         &
% % 	   	x.xxx                                      &
% % 	   	Student                                    &
% % 	   	xxx                                        &
% % 	    xxx (s)	                                   &
% % 	      xxx$\times$                                \\
% % 	   	\cdashline{2-7}                
% %                                                       &
% % 	   	\multirow{3}{*}{Few-shot meta-predictor}   &
% % 	   	0.553                                      &
% % 	   	Student                                    &
% % 	   	5                                          &
% % 	    4069.585 (s)	                                   &
% % 	      xxx$\times$                                \\
% % 	   	                                          &
% % 	   	                                          &
% % 	   	0.549                                      &
% % 	   	Student                                    &
% % 	   	3                                          &
% % 	    2441.751 (s)	                                   &
% % 	      xxx$\times$                                \\
% % 	   	                                          &
% % 	   	                                          &
% % 	   	0.590                                      &
% % 	   	Student                                    &
% % 	   	1                                          &
% % 	    813.917 (s)	                                   &
% % 	      xxx$\times$                                \\
% % 	   	\cdashline{2-7}                    	
% % 	   	                                        &
% % 	   	\textbf{Ours}                              &
% % 	   	0.731                                      &
% % 	   	Teacher                                    &
% % 	   	1                                          &
% % 	    xxx (s)	                                   &
% % 	      xxx$\times$                                \\
% % 	   	\midrule
%             \multicolumn{1}{c}{\multirow{4}{*}{STL10}}    &
% 	   	\multicolumn{1}{c}{\multirow{3}{*}{Few-shot meta-prediction model}}   &
% 	   	0.297                                      &
% 	   	Student                                    &
% 	   	5                                          &
% 	    4303.89 (s)	                                   &
% 	      1.000$\times$                                \\
% 	   	                                       &
% 	   	                                          &
% 	   	0.267                                     &
% 	   	Student                                    &
% 	   	3                                          &
% 	    2582.33 (s)	                                   &
% 	    1.667$\times$                                \\
% 	   	                                         &
% 	   	                                          &
% 	   	0.219                                      &
% 	   	Student                                    &
% 	   	1                                          &
% 	    860.777 (s)	                                   &
% 	      5.000$\times$                                \\
% 	   	\cdashline{2-7}     
% 	   	%\midrule
% 	   	                                       &
% 	   	\multicolumn{1}{c}{\textbf{Ours}}                              &
% 	   	0.485                                      &
% 	   	Teacher                                    &
% 	   	1                                          &
% 	    4.654 (s)	                                   &
% 	      924.771$\times$                                \\
% % %%%%%%%%%%%%%%%%%%%%%%%%   Stanford Dogs  %%%%%%%%%%%%%%%%%%%%%%%%%
% %             \multirow{6}{*}{Stanford Dogs}                  &
% % 	   	\multirow{2}{*}{Task-specific predictor}   &
% % 	   	x.xxx                                      &
% % 	   	Student                                    &
% % 	   	xxx                                        &
% % 	    xxx (s)	                                   &
% % 	      xxx$\times$                                \\
% %                                                         &
% %                                                         &
% % 	   	x.xxx                                      &
% % 	   	Student                                    &
% % 	   	xxx                                        &
% % 	    xxx (s)	                                   &
% % 	      xxx$\times$                                \\
% % 	   	\cdashline{2-7}                
% %                                                       &
% % 	   	\multirow{3}{*}{Few-shot meta-predictor}   &
% % 	   	0.422                                      &
% % 	   	Student                                    &
% % 	   	5                                          &
% % 	    8228.820 (s)	                                   &
% % 	      xxx$\times$                                \\
% % 	   	                                          &
% % 	   	                                          &
% % 	   	0.447                                      &
% % 	   	Student                                    &
% % 	   	3                                          &
% % 	    4937.292 (s)	                                   &
% % 	      xxx$\times$                                \\
% % 	   	                                          &
% % 	   	                                          &
% % 	   	0.414                                      &
% % 	   	Student                                    &
% % 	   	1                                          &
% % 	    1645.764 (s)	                                   &
% % 	      xxx$\times$                                \\
% % 	   	\cdashline{2-7}                    	
% % 	   	                                        &
% % 	   	\textbf{Ours}                              &
% % 	   	0.578                                      &
% % 	   	Teacher                                    &
% % 	   	1                                          &
% % 	    xxx (s)	                                   &
% % 	      xxx$\times$                                \\
% % 	   	\midrule
% % %%%%%%%%%%%%%%%%%%%%%%%%   DTD  %%%%%%%%%%%%%%%%%%%%%%%%%
% %             \multirow{6}{*}{DTD}                  &
% % 	   	\multirow{2}{*}{Task-specific predictor}   &
% % 	   	x.xxx                                      &
% % 	   	Student                                    &
% % 	   	xxx                                        &
% % 	    xxx (s)	                                   &
% % 	      xxx$\times$                                \\
% %                                                         &
% %                                                         &
% % 	   	x.xxx                                      &
% % 	   	Student                                    &
% % 	   	xxx                                        &
% % 	    xxx (s)	                                   &
% % 	      xxx$\times$                                \\
% % 	   	\cdashline{2-7}                
% %                                                       &
% % 	   	\multirow{3}{*}{Few-shot meta-predictor}   &
% % 	   	0.334                                      &
% % 	   	Student                                    &
% % 	   	5                                          &
% % 	    3150.475 (s)	                                   &
% % 	      xxx$\times$                                \\
% % 	   	                                          &
% % 	   	                                          &
% % 	   	0.340                                      &
% % 	   	Student                                    &
% % 	   	3                                          &
% % 	    1890.285 (s)	                                   &
% % 	      xxx$\times$                                \\
% % 	   	                                          &
% % 	   	                                          &
% % 	   	0.312                                      &
% % 	   	Student                                    &
% % 	   	1                                          &
% % 	    630.095 (s)	                                   &
% % 	      xxx$\times$                                \\
% % 	   	\cdashline{2-7}                    	
% % 	   	                                        &
% % 	   	\textbf{Ours}                              &
% % 	   	0.401                                      &
% % 	   	Teacher                                    &
% % 	   	1                                          &
% % 	    xxx (s)	                                   &
% % 	      xxx$\times$                                \\
% % 	   	\midrule
% % %%%%%%%%%%%%%%%%%%%%%%%%   CIFAR-10  %%%%%%%%%%%%%%%%%%%%%%%%%
% %             \multirow{6}{*}{CIFAR-10}                  &
% % 	   	\multirow{2}{*}{Task-specific predictor}   &
% % 	   	x.xxx                                      &
% % 	   	Student                                    &
% % 	   	xxx                                        &
% % 	    xxx (s)	                                   &
% % 	      xxx$\times$                                \\
% %                                                         &
% %                                                         &
% % 	   	x.xxx                                      &
% % 	   	Student                                    &
% % 	   	xxx                                        &
% % 	    xxx (s)	                                   &
% % 	      xxx$\times$                                \\
% % 	   	\cdashline{2-7}                
% %                                                       &
% % 	   	\multirow{3}{*}{Few-shot meta-predictor}   &
% % 	   	0.430                                      &
% % 	   	Student                                    &
% % 	   	5                                          &
% % 	    32382.180 (s)	                                   &
% % 	      xxx$\times$                                \\
% % 	   	                                          &
% % 	   	                                          &
% % 	   	0.422                                      &
% % 	   	Student                                    &
% % 	   	3                                          &
% % 	    19429.308 (s)	                                   &
% % 	      xxx$\times$                                \\
% % 	   	                                          &
% % 	   	                                          &
% % 	   	0.382                                      &
% % 	   	Student                                    &
% % 	   	1                                          &
% % 	    6476.436 (s)	                                   &
% % 	      xxx$\times$                                \\
% % 	   	\cdashline{2-7}                    	
% % 	   	                                        &
% % 	   	\textbf{Ours}                              &
% % 	   	0.374                                      &
% % 	   	Teacher                                    &
% % 	   	1                                          &
% % 	    xxx (s)	                                   &
% % 	      xxx$\times$                                \\
% % 	   	\midrule
% %%%%%%%%%%%%%%%%%%%%%%%%   CIFAR-100  %%%%%%%%%%%%%%%%%%%%%%%%%
%             % \multicolumn{1}{c}{\multirow{4}{*}{CIFAR-100}}                  &
% 	   %	\multicolumn{1}{c|}{\multirow{2}{*}{Task-specific predictor}}   &
% 	   %	x.xxx                                      &
% 	   %	Student                                    &
% 	   %	xxx                                        &
% 	   % xxx (s)	                                   &
% 	   %   xxx$\times$                                \\
%     %                                                     &
%     %                                                     &
% 	   %	x.xxx                                      &
% 	   %	Student                                    &
% 	   %	xxx                                        &
% 	   % xxx (s)	                                   &
% 	   %   xxx$\times$                                \\
% 	   %	\cdashline{2-7}       
% 	   %%\midrule
%     %                                                   &
% 	   %	\multicolumn{1}{c|}{\multirow{3}{*}{Few-shot meta-predictor}}   &
% 	   % \multicolumn{1}{c}{\multirow{4}{*}{CIFAR-100}}    &
% 	   % 	\multicolumn{1}{c|}{\multirow{3}{*}{Few-shot meta-predictor}}   &
% 	   % 	0.250                                      &
% 	   % 	Student                                    &
% 	   % 	5                                          &
% 	   %  32171.220 (s)	                                   &
% 	   %    1.000$\times$                                \\
% 	   % 	                                       &
% 	   % 	                                          &
% 	   % 	0.212                                      &
% 	   % 	Student                                    &
% 	   % 	3                                          &
% 	   %  19302.732 (s)	                                   &
% 	   %  1.667$\times$                                \\
% 	   % 	                                         &
% 	   % 	                                          &
% 	   % 	0.147                                      &
% 	   % 	Student                                    &
% 	   % 	1                                          &
% 	   %  6434.244 (s)	                                   &
% 	   %    5.000$\times$                                \\
% 	   % 	\cdashline{2-7}     
% 	   % 	%\midrule
% 	   % 	                                       &
% 	   % 	\multicolumn{1}{c|}{\textbf{Ours}}                              &
% 	   % 	0.406                                      &
% 	   % 	Teacher                                    &
% 	   % 	1                                          &
% 	   %  4.101 (s)	                                   &
% 	   %    7844.726$\times$                                \\
% % 	   	\midrule     
% % %%%%%%%%%%%%%%%%%%%%%%%%   STL10  %%%%%%%%%%%%%%%%%%%%%%%%%
% %             \multirow{6}{*}{STL10}                  &
% % 	   	\multirow{2}{*}{Task-specific predictor}   &
% % 	   	x.xxx                                      &
% % 	   	Student                                    &
% % 	   	xxx                                        &
% % 	    xxx (s)	                                   &
% % 	      xxx$\times$                                \\
% %                                                         &
% %                                                         &
% % 	   	x.xxx                                      &
% % 	   	Student                                    &
% % 	   	xxx                                        &
% % 	    xxx (s)	                                   &
% % 	      xxx$\times$                                \\
% % 	   	\cdashline{2-7}                
% %                                                       &
% % 	   	\multirow{3}{*}{Few-shot meta-predictor}   &
% % 	   	0.220                                      &
% % 	   	Student                                    &
% % 	   	5                                          &
% % 	    4303.885 (s)	                                   &
% % 	      xxx$\times$                                \\
% % 	   	                                          &
% % 	   	                                          &
% % 	   	0.216                                      &
% % 	   	Student                                    &
% % 	   	3                                          &
% % 	    2582.331 (s)	                                   &
% % 	      xxx$\times$                                \\
% % 	   	                                          &
% % 	   	                                          &
% % 	   	0.158                                      &
% % 	   	Student                                    &
% % 	   	1                                          &
% % 	    860.777 (s)	                                   &
% % 	      xxx$\times$                                \\
% % 	   	\cdashline{2-7}                    	
% % 	   	                                        &
% % 	   	\textbf{Ours}                              &
% % 	   	0.320                                      &
% % 	   	Teacher                                    &
% % 	   	1                                          &
% % 	    xxx (s)	                                   &
% % 	      xxx$\times$                                \\
% 	   	\bottomrule
%         \end{tabular}
% 	    }
% 	\end{center}
% 	\small

% 	\vspace{-0.1in}
% \end{table*}


\vspace{-0.1in}
\begin{table}[h]

\centering
\caption{\small \textbf{Efficacy and Sample Efficiency of the Proposed Meta-prediction Model for DaNAS} \small Comparison of the Spearman's rank correlation coefficient (\textbf{Corr.}) and the time required to collect samples for adaptation in guided search (\textbf{Collecting Time}).}
\label{tbl:time}
\vspace{-0.1in}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccccc}
\toprule
\multirow{2}{*}{Target Dataset} & \multirow{2}{*}{Method}                         & \multirow{2}{*}{Corr.} & \multicolumn{4}{c}{Training}    \\
 &      &       & Sample Type & \# of Samples & Collecting Time (s) & Speed Up  \\ \midrule \midrule
\multirow{4}{*}{STL}            & \multirow{3}{*}{Few-shot meta-prediction model} & 0.297                  & Student & 5 & 4303.89 & 1.000 × \\
 &      & 0.267 & Student     & 3             & 2582.33             & 1.667 x   \\
 &      & 0.219 & Student     & 1             & 860.78              & 5.000 x   \\ \vspace{0.01in}\cdashline{2-7}
 & \textbf{Ours} & 0.485 & Teacher     & 1             & 4.65                & \textbf{924.771 x} \\ \bottomrule
\end{tabular}%
}
\vspace{-0.1in}
\end{table}
